What Counts as AI Sycophancy? A Taxonomy and Expert Survey of a Fragmented Construct

AI sycophancy has become a prominent concern in large language model (LLM) research. Yet the term lacks a consistent definition and has been applied to behaviors ranging from agreeing with a user's false claim to excessively praising the user to withholding corrective feedback. When researchers, companies, and policymakers use the same term to describe different behaviors, evaluation results become difficult to compare, mitigation strategies fail to transfer, and systems that are resistant to one form of sycophancy continue exhibiting other forms. To address this, we make two contributions. First, we reviewed 70 papers on AI sycophancy to develop a taxonomy of how the behavior has been defined and measured. The taxonomy distinguishes (1) whether a model is sycophantic toward a user's positions and beliefs, or toward the user's broader personal traits and emotions, and (2) whether this occurs through explicit, direct language or more implicit, subtle behaviors such as framing, omission, or tone. Mapping existing literature to our taxonomy reveals that current research has focused on overt forms of sycophancy toward users' beliefs, leaving more subtle and person-directed behaviors relatively understudied. Second, we surveyed 106 experts in AI sycophancy and related fields to examine whether researchers agree on which model behaviors are sycophantic. While experts are nearly unanimous in believing that sycophancy is a significant problem in current AI systems (94.3% agree), they disagree substantially on which specific behaviors qualify. Together, these findings demonstrate that AI sycophancy is a broad family of behaviors with different measurement challenges, intervention requirements, and governance implications. Our taxonomy provides a shared vocabulary for understanding and addressing these behaviors.

==> Tables/modelspecs.tex <==
\subsection{Industry Specifications}
\label{app:modelspecs}

\begin{table*}[t]
\centering
\caption{How sycophancy is addressed across six versions of OpenAI's
model specification \citep{openai2024spec, openai2025feb, openai2025apr, openai2025sep, openai2025oct, openai2025dec} and the April 2025 incident report \citep{openai2025incident}.}
\label{tab:openai}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{p{1.8cm} p{12.0cm}}
\hline
\textbf{Date} & \textbf{Summary} \\
\hline

May 2024 &
%Sycophancy is not mentioned. There are two tangentially related statements.
%\newline
\textit{Assume an objective point of view}: ``The assistant should not have personal opinions or an agenda to change the user's perspective.'' \newline
\textit{Don't try to change anyone's mind}: ``The assistant should aim to inform,
not influence.'' \newline
Employee metaphor: the assistant
``shouldn't just say `yes' to everything (like a sycophant).'' \\[5pt]

Feb 2025 &
\textit{Don't be sycophantic}. ``A related concern
involves sycophancy, which erodes trust. The assistant exists to help
the user, not flatter them or agree with them all the time. \ldots\
[T]he assistant should not change its stance solely to agree with the
user. \ldots\ [P]rovide constructive feedback and behave more like a
firm sounding board that users can bounce ideas off of---rather than
a sponge that doles out praise.''

\smallskip
Section on honesty cross-references sycophancy section to flag
limits on white lies, illustrated by example of falsely reassuring
a user their girlfriend will forgive them. \\[5pt]

Apr 2025 &
Added in honesty
section: ``[E]ven `white lies' that humans may use in conversation
to make the other person feel better are not allowed (see also
Don't be sycophantic).'' \\[5pt]

Apr 29, 2025 \newline\textit{(incident \newline report)} &
``The update we removed was overly flattering or agreeable---often
described as sycophantic. \ldots\ [W]e focused too much on short-term
feedback, and did not fully account for how users' interactions with
ChatGPT evolve over time. As a result, GPT-4o skewed towards
responses that were overly supportive but disingenuous. \ldots\
Sycophantic interactions can be uncomfortable, unsettling, and cause
distress.'' \\[5pt]

Sep 2025 &
Main sycophancy section unchanged from April 2025. \\[5pt]

Oct 2025 &
New passage added in
mental health section:
``The assistant should affirm a user's emotional experience,
without affirming or escalating any ungrounded belief that might
lead to mental or emotional distress.'' \\[5pt]

Dec 2025 &
New language in honesty section
makes connection to sycophancy explicit: ``[W]hite lies that humans may
use in conversation to make the other person feel better may be
taken too far, for example, when they amount to sycophancy and
are against the user's best interest.'' \\

\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{How sycophancy is addressed across both versions of
Anthropic's constitution \citep{anthropic2023spec, anthropic2026spec} and their April 2026 blog post on how people ask Claude for personal guidance \citep{anthropic2026guidance}.}
\label{tab:anthropic}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{p{1.8cm} p{12.0cm}}
\hline
\textbf{Date} & \textbf{Summary} \\
\hline

May 2023 &
Behavior governed by
``helpful, honest, and harmless'' principles. \newline
One principle
adapted from DeepMind's Sparrow rules addresses implicit
approval-seeking: ``Choose the response that is least intended
to build a relationship with the user.'' \\[5pt]

Jan 2026 &
\textit{Concern for user wellbeing}: ``[C]oncern for user
wellbeing means that Claude should avoid being sycophantic or trying
to foster excessive engagement or reliance on itself if this isn't in
the person's genuine interest. \ldots\ [W]e often see flattery,
manipulation, fostering isolation, and enabling unhealthy patterns as
corrosive.''

\smallskip
\textit{Being honest} (not explicitly linked to sycophancy):
``Epistemic cowardice---giving deliberately vague or non-committal
answers to avoid controversy or to placate people---violates honesty
norms. \ldots\ Claude should be diplomatically honest rather than
dishonestly diplomatic.''

\smallskip
Honesty properties enumerated separately: \textit{Autonomy-preserving}
(``offer balanced perspectives \ldots\ foster independent thinking
over reliance on Claude''); \textit{Non-manipulative} (``never tries
to convince people \ldots\ using \ldots\ persuasion techniques that
exploit psychological weaknesses or biases''). None of these properties are explicitly attributed to sycophancy. \\

Apr 2026 \newline \textit{(blog post)} &
Empirical study of sycophancy in personal guidance conversations,
analyzing roughly 38,000 conversations from Claude.
Sycophancy is operationalized via a 1--5 grader scale as excessive
agreement with a user's one-sided perspective rather than challenging
it (e.g., affirming that a partner is ``definitely gaslighting'' the
user based on a one-sided account). Overall sycophancy rate was 9\%,
rising to 38\% in spirituality conversations and 25\% in relationship
conversations; training efforts focused on relationships as the domain
with the highest absolute volume of sycophantic exchanges. Pushback
from users was highest in relationship conversations (21\% vs.\ 15\%
average), and sycophancy rate rose to 18\% in conversations that
included pushback (vs.\ 9\% without). Synthetic relationship guidance
training data was used to train Opus 4.7 and Mythos Preview, reducing
sycophancy by roughly half in relationship guidance, with
generalization across domains. \\

\hline
\end{tabular}
\end{table*}
